Few-Shot Self-Rationalization with Natural Language Prompts

Self-rationalization models that predict task labels and generate free-text elaborations for their predictions could enable more intuitive interaction with NLP systems. These models are, however, currently trained with a large amount of human-written free-text explanations for each task which hinders their broader usage. We propose to study a more realistic setting of self-rationalization using few training examples. We present FEB -- a standardized collection of four existing English-language datasets and associated metrics. We identify the right prompting approach by extensively exploring natural language prompts on FEB. Then, by using this prompt and scaling the model size, we demonstrate that making progress on few-shot self-rationalization is possible. We show there is still ample room for improvement in this task: the average plausibility of generated explanations assessed by human annotators is at most 51% (with GPT-3), while plausibility of human explanations is 76%. We hope that FEB and our proposed approach will spur the community to take on the few-shot self-rationalization challenge.

==> figs/gpt3.tex <==
\begin{figure}[t]
    \begin{tcolorbox}[width=\columnwidth, colframe=gray!20, colback=gray!10, halign=left, boxsep=0pt]
        \small
        \texttt{[Task description]}
        
        \texttt{[Input Type1]: [Input1]}
        
        \texttt{[Input Type2]: [Input2]}
        
        \texttt{Answer: [Label]}
        
        \texttt{Reason: [Explanation]}
    \end{tcolorbox}
    \caption{GPT-3 prompt template for all datasets. 
    The strings \texttt{[Task description]}, \texttt{[Input Type1]}, and \texttt{[Input Type2]} depend on the task. Check Appendix for the detailed prompts. }
\label{fig:gpt3_prompt}
\end{figure}

==> tables/prompts_esnli.tex <==
\begin{table*}[t]
 \resizebox{\textwidth}{!}{  
 \centering
\begin{tabular}{llp{10.5cm}p{6.5cm}}
\toprule
\textbf{Type} & \textbf{Id} & \textbf{Input} & \textbf{Output}\\
\midrule
\multirow{4}{*}{\footnotesize \textsc{MASK}} & 1 & explain nli hypothesis: [hypothesis] premise: [premise] \textless{}extra\_id\_0\textgreater{} because \textless{}extra\_id\_1\textgreater{}{} & \textless{}extra\_id\_0\textgreater{}  [label] \textless{}extra\_id\_1\textgreater{} [explanation] \textless{}extra\_id\_2\textgreater{}{} \\
 & 2 & explain nli hypothesis: [hypothesis] premise: [premise] The entailment relation is \textless{}extra\_id\_0\textgreater{} because \textless{}extra\_id\_1\textgreater{}{} & \textless{}extra\_id\_0\textgreater{}  [label] \textless{}extra\_id\_1\textgreater{} [explanation] \textless{}extra\_id\_2\textgreater{}{} \\
\midrule
\textsc{\footnotesize $\sim$T5 \textsc{(MNLI)}} & 3 &  explain nli hypothesis: [hypothesis] premise: [premise] & [label] because [explanation] \\
\midrule
\multirow{7}{*}{\footnotesize \textsc{QA}$\times$\textsc{SQuAD-T5}} & 4 &  explain nli question: Does premise entail hypothesis? context: [hypothesis] [premise] & [yes/no/maybe] because [explanation] \\
* & 5 &  explain nli question: What is this? context: [hypothesis] [premise] & [label] because [explanation]  \\
* & 6 &  explain nli question: Does premise entail hypothesis? context: hypothesis: [hypothesis] premise: [premise] & [yes/no/maybe] because [explanation] \\
* & 7 &  explain nli question: What is this? context: hypothesis: [hypothesis] premise: [premise] & [label] because [explanation] \\
\arrayrulecolor{black!20}\midrule
\multirow{11}{*}{\footnotesize \textsc{QA}$\times$\textsc{UnifiedQA}} & 8 &  EXPLAIN [premise] IS [hypothesis]? \textbackslash{}\textbackslash{} (A) Yes, (B) Maybe, (C) No & [yes/no/maybe] BECAUSE [explanation] \\
 & 9 & EXPLAIN premise: [premise] IS hypothesis: [hypothesis]? \textbackslash{}\textbackslash{} (A) Yes, (B) Maybe, (C) No & [yes/no/maybe] BECAUSE [explanation] \\
  & 10 & EXPLAIN Does premise entail hypothesis? \textbackslash{}\textbackslash{}{}n [hypothesis] [premise] & [yes/no/maybe] BECAUSE [explanation] \\
 & 11 & EXPLAIN Does premise entail hypothesis? \textbackslash{}\textbackslash{}{}n hypothesis: [hypothesis] premise: [premise] & [yes/no/maybe] BECAUSE [explanation] \\
 & 12 & EXPLAIN Does premise entail hypothesis? \textbackslash{}\textbackslash{}{}n (A) Yes, (B) Maybe, (C) No \textbackslash{}\textbackslash{}{}n hypothesis: [hypothesis] premise: [premise] & [yes/no/maybe] BECAUSE [explanation] \\
  &13 &  EXPLAIN What is this? \textbackslash{}\textbackslash{}{}n [hypothesis] [premise] & [label] BECAUSE [explanation] \\
 &14 &  EXPLAIN What is this? \textbackslash{}\textbackslash{}{}n hypothesis: [hypothesis] premise: [premise] & [label] BECAUSE [explanation] \\
 & 15 & EXPLAIN What is this? \textbackslash{}\textbackslash{}{}n (A) entailment, (B) neutral, (C) contradiction \textbackslash{}\textbackslash{}{}n hypothesis:  [hypothesis] premise: [premise]  & [label] BECAUSE [explanation]  \\
\arrayrulecolor{black}\bottomrule
\end{tabular}
}
\caption{Prompts for self-rationalization in \textsc{E-SNLI}. ``\textsc{MASK}'' marks span-filling prompts; ``$\sim$T5'' marks prompts following the most similar T5 pretraining task; ``\textsc{QA$\times$SQuAD-T5}'' marks the QA prompt following \textsc{SQuAD}'s formatting for T5 pretraining; and ``\textsc{QA$\times$UnifiedQA}'' marks QA prompts following \textsc{UnifiedQA}.}
\label{prompts:e_snli}
\end{table*}

==> tables/results_scale_model_size.tex <==
\begin{table}[t]
\centering
 \resizebox{\columnwidth}{!}{  
\begin{tabular}{llrrr}
\toprule
& \textbf{Size} & \textbf{Accuracy}  & \textbf{BERTscore} & \textbf{Plausibility} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{E-SNLI}}} & \textsc{\small Base} & 79.21$_{0.29}$ & 71.34$_{0.27}$ & 16.75$_{1.53}$\\
                      &\textsc{\small Large} & 84.79$_{0.27}$ &	76.56$_{0.27}$ & 32.68$_{1.92}$ \\
                      &\textsc{\small 3B} & \textbf{87.43}$_{0.23}$ & \textbf{79.10}$_{0.23}$ & 41.60$_{2.08}$ \\
                      %&\textsc{\small 11B} & & & \\ 
\arrayrulecolor{black!20}\cmidrule{2-5}
%                      &\textsc{\small GPT-3} & 65.37$_{4.10}$ & 59.83$_{3.67}$  & \\
                      &\textsc{\small GPT-3} & 65.37$_{0.53}$ & 59.83$_{0.47}$  & \textbf{42.44}$_{2.17}$ \\
\arrayrulecolor{black!20}\cmidrule{2-5}
&\textsc{\small Gold} & \makecell[c]{-} & \makecell[c]{-} & 77.40$_{1.59}$  \\
\arrayrulecolor{black!20}\cmidrule{2-5}
&\textsc{\small Random} & \makecell[c]{33.33} & \makecell[c]{-} &  \makecell[c]{-} \\
\arrayrulecolor{black}\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{ECQA}}} & \textsc{\small Base}  & 41.37$_{0.34}$ & 36.72$_{0.30}$ & 25.52$_{1.25}$\\
                      &\textsc{\small Large} & 57.19$_{0.36}$ &	51.00$_{0.32}$ &  \ana{tbd}\\
                      &\textsc{\small 3B} & \textbf{65.86}$_{0.36}$ & \textbf{58.98}$_{0.32}$ &\ana{tbd} \\
                     %& \textsc{\small 11B} & & & \\
\arrayrulecolor{black!20}\cmidrule{2-5}
%                      &\textsc{\small GPT-3} & 60.65$_{11.44}$ & 54.42$_{10.23}$ & \\
                      &\textsc{\small GPT-3} & 60.65$_{1.48}$ & 54.42$_{1.32}$ & 45.06$_{1.44}$\\
\arrayrulecolor{black!20}\cmidrule{2-5}                      
                    &\textsc{\small Gold} & \makecell[c]{-} & \makecell[c]{-} & \ana{tbd}   \\
\arrayrulecolor{black!20}\cmidrule{2-5}
&\textsc{\small Random} & \makecell[c]{20.00} & \makecell[c]{-} &  \makecell[c]{-} \\
\arrayrulecolor{black}\midrule
\multirow{6}{*}{\rotatebox{90}{\textsc{ComVE}}} & \textsc{\small Base}  & 67.33$_{0.71}$ &	60.97$_{0.64}$ & 13.80$_{1.26}$\\
                     & \textsc{\small Large} & 81.31$_{0.39}$ &	73.95$_{0.36}$ & 25.59$_{1.67}$ \\
                     & \textsc{\small 3B} & \textbf{88.96}$_{0.38}$ & \textbf{81.02}$_{0.34}$ & 33.40$_{1.71}$\\
                     %& \textsc{\small 11B} & & & \\ 
\arrayrulecolor{black!20}\cmidrule{2-5}
%                      &\textsc{\small GPT-3} & 73.98$_{10.81}$ & 67.65$_{10.0}$ & \textbf{42.16}$_{34.19}$\\
                      &\textsc{\small GPT-3} & 73.98$_{1.40}$ & 67.65$_{1.29}$ & \textbf{42.16}$_{1.80}$\\
\arrayrulecolor{black!20}\cmidrule{2-5}
                      &\textsc{\small Gold} & \makecell[c]{-} & \makecell[c]{-} & 77.24$_{1.30}$\\
\arrayrulecolor{black!20}\cmidrule{2-5}
&\textsc{\small Random} & \makecell[c]{50.00} & \makecell[c]{-} &  \makecell[c]{-} \\
\arrayrulecolor{black}\midrule                    
\multirow{6}{*}{\rotatebox{90}{\textsc{SBIC}}} & \textsc{\small Base}  & 67.55$_{0.41}$ &	65.29$_{0.39}$ &  57.96$_{2.25}$\\
                     & \textsc{\small Large} & 71.06$_{0.39}$ &	68.55$_{0.39}$ & 61.82$_{2.23}$ \\
                     & \textsc{\small 3B} & 71.66$_{0.48}$ & 68.90$_{0.49}$ & 64.20$_{2.14}$\\
                    %&  \textsc{\small 11B} & & & \\ 
                    \arrayrulecolor{black!20}\cmidrule{2-5}
%                    &\textsc{\small GPT-3} & \textbf{74.17}$_{10.96}$ & \textbf{71.53}$_{10.85}$ & \textbf{72.68}$_{32.71}$ \\
                    &\textsc{\small GPT-3} &  \textbf{74.17}$_{1.41}$ & \textbf{71.53}$_{1.40}$ & \textbf{72.68}$_{1.72}$ \\
\arrayrulecolor{black!20}\cmidrule{2-5}
                    &\textsc{\small Gold} & \makecell[c]{-} & \makecell[c]{-} & 79.81$_{1.62}$ \\ 
\arrayrulecolor{black!20}\cmidrule{2-5}
&\textsc{\small Random} & \makecell[c]{50.00} & \makecell[c]{-} &  \makecell[c]{-} \\
\arrayrulecolor{black}\bottomrule
\end{tabular}}
\caption{Self-rationalization w.r.t.\ the model's size. \ana{Move comparison with GPT-3 to a new table because accuracy and bertscore for other models are calculated wtih 60 train-dev splits and we can't afford 60*350*4 GPT-3 inferences so we'll report GPT-3 results on a single train-dev split?}
\ib{which model is used for the base,large,3b,11b runs?}}
\label{tab:scale_size}
\end{table}

==> tables/results_unifiedqa_vs_squad.tex <==
\begin{table}[t]
\centering
 \resizebox{\columnwidth}{!}{ 
\begin{tabular}{lcccc}
\toprule      
          & \esnli   & \ecqa        & \comve          & \sbic           \\
\midrule
\textsc{\small UniQA} & 75.05$_{0.34}$ & \textbf{41.37}$_{0.34}$  & \textbf{67.33}$_{0.71}$ & \textbf{67.55}$_{0.41}$ \\
{\small T5}        & \textbf{77.86}$_{0.34}$ & 36.48$_{0.34}$   & 54.49$_{0.46}$ & 66.99$_{0.53}$ \\
\bottomrule
\toprule
          & \esnli   & \ecqa       & \comve          & \sbic           \\
\midrule
\textsc{\small UniQA}  & 67.52$_{0.33}$ & \textbf{36.72}$_{0.30}$ & \textbf{60.97}$_{0.64}$ & \textbf{65.29}$_{0.39}$\\
{\small T5}        & \textbf{70.08}$_{0.32}$ & 32.38$_{0.30}$ & 49.25$_{0.42}$ & 64.60$_{0.56}$ \\
\bottomrule
\end{tabular}
}
\caption{A comparison of \unifiedqa and T5 when prompted with nearly identical  \unifiedqaprompt and \squadprompt prompts, respectively. The upper part shows accuracy and the lower part BERTscore. See \sect{sec:qa_prompts} for descriptions of these prompts.}
\label{tab:unifiedqa_vs_squad}
\end{table}

==> tables/tasks_and_similar_tasks.tex <==
\newcolumntype{?}{!{\vrule width 2pt}}

\begin{table*}[!ht]
 \resizebox{\textwidth}{!}{  
\begin{tabular}{lp{5cm}c?lp{5cm}}
\toprule
\multicolumn{2}{l}{\textbf{\benchmark Tasks}}   & \textbf{\# Shots} & \multicolumn{2}{l}{\textbf{Similar T5 Pretraining Tasks}} \\
\midrule
\makecell[tl]{\textsc{E-SNLI}\\ \cite{camburu2018snli}} & Classify the entailment relation between two sequences & 16 & \makecell[tl]{\textsc{MNLI}\\  \cite{williams-etal-2018-broad}}  & Classify the entailment relation between two sequences                    \\
\arrayrulecolor{black!20}\midrule
\makecell[tl]{\textsc{ECQA}\\ \cite{aggarwal-etal-2021-explanations}} & Answer a question,  given five answer choices & 48     & \makecell[tl]{\textsc{RECORD}\\ \cite{Zhang2018ReCoRDBT}} & Answer a cloze-style query about a passage given entities in it         \\
\arrayrulecolor{black!20}\midrule
\makecell[tl]{\textsc{ComVE}\\ \cite{wang-etal-2019-make}}  & Select one of two sequences as more nonsensical & 24 & \makecell[tl]{\textsc{COPA}\\ \cite{Roemmele2011COPA}}  & Select one of two sequences as the cause/effect of a premise \\
\arrayrulecolor{black!20}\midrule
\makecell[tl]{\textsc{SBIC}\\ \cite{sap-etal-2020-social}} & Classify a post as offensive or not & 24   & \makecell[tl]{\textsc{COLA}\\  \cite{warstadt-etal-2019-neural}}  & Classify a sentence as acceptable or not       \\
\arrayrulecolor{black}\bottomrule
\end{tabular}
}
\caption{The left part of the table shows tasks that we have included in \benchmark. Tasks on the right are included in T5's pretraining and they are similar to \benchmark's tasks. We explore self-rationalization prompts for \benchmark's tasks based on the tasks on the right, and compare them to prompts designed as span infilling and QA  (\sect{sec:study_various_prompts}). 
}
\label{tab:tasks}
\end{table*}
